FlexSA: Flexible Systolic Array Architecture for Efficient Pruned DNN Model Training

Modern deep learning models have high memory and computation cost. To make them fast and memory-cost efficient, structured model pruning is commonly used. We find that pruning a model using a common training accelerator with large systolic arrays is extremely performance-inefficient. To make a systolic array efficient for pruning and training, we propose FlexSA, a flexible systolic array architecture. FlexSA dynamically reconfigures the systolic array structure and offers multiple sub-systolic operating modes, which are designed for energy- and memory bandwidth-efficient processing of tensors with different sizes and shapes. We also present a compilation heuristic for tiling matrix-multiplication-and-accumulation operations in a training workload to best utilize the resources of FlexSA. Based on our evaluation, FlexSA with the proposed compilation heuristic improves compute resource utilization of pruning and training modern CNN models by 37% compared to a conventional training accelerator with a large systolic array. FlexSA also improves on-chip data reuse by 1.7X saving 28% energy compared to naive systolic array splitting.

==> Makefile <==
all:  main.tex bib/*.bib IEEEtran.cls
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex -synctex=-1 main
	#sed -i -e 's/build_tex/tex/g' -e 's/\/cygdrive\/c/C:/g' main.synctex
	#gs -sOutputFile=main_bw.pdf -sDEVICE=pdfwrite -sColorConversionStrategy=Gray -dProcessColorModel=/DeviceGray -dCompatibilityLevel=1.4 -dNOPAUSE -dBATCH main.pdf
clean: 
	rm -rf *.aux *.bbl *.blg *.log *.out main.pdf main_bw.pdf main.dvi main.synctex


==> tex/eval_old.tex <==
%\section{Evaluation}
%\label{sec:flexsa_evaluation}

\section{Evaluation Methodology and \\Baseline Scheduling Policy}
\label{sec:flexsa_evaluation_method}

We develop an instruction-level architecture simulator to evaluate the performance and energy efficiency of our proposed ides. We use ResNet50, the most commonly used CNN model for various vision tasks, for pruning and retraining. We also use Inception v4~\cite{szegedy2017inception}, though only artificially pruning the model by applying the same pruning statistics of ResNet50. We use PruneTrain as the pruning mechanism, with two different model-pruning strengths as shown in \sect{sec:flexsa_motivation}. The model is trained for 90 epochs with a pruning interval of 10 epochs and the mini-batch size of 32 per processor. We use mixed-precision multiplication and accumulation~\cite{micikevicius2017mixed} to execute the GEMMs of the convolution and FC layers.

In our evaluation, five different accelerator configurations are used, as summarized in \tab{tab:flexsa_config}. The {\bf{1G1C}} configuration uses a single 128$\times$128 systolic array, {\bf{1G4G}} splits this large core into four 64$\times$64 cores, which share a single GBUF. The {\bf{4G4C}} configuration further splits the cores into 16 32$\times$32 cores, where we divide the cores and the GBUF into four groups with cores in each group sharing a GBUF. The {\bf{1G1F}} configuration has a single 128$\times$128 FlexSA with four 64$\times$64 cores, and {\bf{4G1F}} has four small FlexSAs, each with a dedicated GBUF. We use a GBUF size of 10MB as used in WaveCore~\cite{lym2018mini} for all core configurations, and a single 270GB/s HBM2 chip as the memory system~\cite{jedec2016hbm2}. All local input and output buffers are sized to support input and output double buffering. The local input buffers holding the horizontally shifted inputs are 2$\times$ larger than the input buffers holding stationary inputs for larger reuse of the pre-loaded stationary inputs. 

\begin{table}[h]
\centering
\caption{Evaluation configuration description.}
    \noindent\resizebox{0.92\linewidth}{!}{
        \begin{tabu}{|[1.2pt]l|l|[1.2pt]}
            \thickhline
            \makecell[c]{Configuration} & \makecell[c]{Description} \tabularnewline
            \midhline
            1G1C                & 1 group each with 1$\times$ (128$\times$128) core \tabularnewline
            \hline
            1G4C                & 1 group each with 4$\times$ (64$\times$64) cores \tabularnewline
            \hline
            4G4C                & 4 groups each with 4$\times$ (32$\times$32) cores \tabularnewline
            \hline
            1G1F           & 1 group each with 4$\times$ (64$\times$64) FlexSA \tabularnewline
            \hline
            4G1F           & 4 groups each with 1$\times$ (32$\times$32) FlexSA \tabularnewline
            \thickhline
        \end{tabu}
    }
    \label{tab:flexsa_config}
\end{table}

DL models contain non-GEMM layers (e.g., feature normalization~\cite{ioffe2015batch,wu2018group}, activation~\cite{nair2010rectified}, and element-wise math layers), which tend to be bound by memory BW. The execution time of these layers changes depending on the accelerator design (off-chip memory BW and on-chip buffer design) and workload scheduling choices (multi-layer fusion~\cite{chen2018tvm} and layer serialization~\cite{alwani2016fused,lym2018mini}). To decouple the impact of such wide variation and concentrate on what we intend to improve with FlexSA, we focus on neuronal (convolution and FC) layer evaluation in this paper.




\medskip
\noindent\textbf{GEMM Partitioning and Blocking.}
The convolution and FC layers have three GEMM execution phases: forward propagation, and data gradient and weight gradient computations in back-propagation. The GEMMs in the forward propagation and data gradient computation are skinny: they have large GEMM height (M), which is the product of the mini-batch and the feature size, and have small GEMM width (N), which is set by the number of output channels. Thus when multiple core groups are used, we partition a GEMM across the M dimension with one partition per core group. On the other hand, the GEMMs for weight gradient computation have small GEMM dimensions in both height and width, but they have large accumulation dimension (K). In this case, we partition the GEMM across the accumulation dimension with one partition per group. Within each GEMM partition, we use 2-level GEMM blocking that holds the inputs of a multiple of GMEM tiles in the GBUF for reuse. Also, within each GEMM partition, each systolic wave is allocated to cores in a group in round-robin fashion for simplicity. When partitioning GEMM across the M dimension, different core groups use the same inputs from the GEMM N dimension. These shared inputs between core groups are replicated to avoid expensive inter-group data transfers. We find that this method efficiently distributes GEMM workloads to multiple cores and core groups.


\section{Evaluation Results}
\label{sec:eval}

\noindent\textbf{PE Utilization and Performance.}
\fig{fig:flexsa_pe_util_ideal} shows the average PE utilization of ResNet50 and Inception v4 across training epochs using different core configurations. This experiment uses infinite (ideal) DRAM BW to isolate the impact on PE utilization to only the size mismatch between systolic waves and cores. Using a single large core (1G1C) shows low PE utilization for both CNNs. The PE utilization of Inception v4 is lower than that of ResNet50 because many of its convolution layers have fewer than 128 channels thus smaller than the height and width of a core. Splitting the core into four small independent cores improves the PE utilization of both CNNs by $\geq$21\% on average as it mitigates internal PE utilization fragmentation. Further splitting a core to sixteen cores improves the PE utilization of both CNNs but with diminishing returns. Using one FlexSA (1G1F) and four small FlexSAs (4G1F) exhibit 0.1\% less ideal PE utilization compared to 1G4C and 4G4C, respectively. Considering that the PE utilization of using independent small cores is the maximum that can be achieved with FlexSA. The result indicates that the FlexSA modes selected by the proposed heuristics achieve near-optimal PE utilization.
%This indicates that the proposed FlexSA mode selection heuristics builds GEMM kernels with optimal PE utilization given the core sizes. Also, in some cases (ResNet50 High and Inception Medium), FlexSA shows higher PE utilization than independent-core design because dividing the GEMMs for weight gradients computation and allocating them to cores leads to uneven GEMM fractions that do not fit core sizes for independent core designs. 

\begin{figure}[t!]
    \centering                                                                            
    \subfloat[Infinite (ideal) DRAM BW]{
        \includegraphics[width=0.48\textwidth]{graphs/pe_util_ideal.pdf}
        \label{fig:flexsa_pe_util_ideal}
    }\\
    \subfloat[Memory system with 1$\times$ HBM2]{
        \includegraphics[width=0.48\textwidth]{graphs/pe_util_hbm.pdf}
        \label{fig:flexsa_pe_util_hbm}
    }
    \caption[PE utilization comparison]{PE utilization and normalized speedup(red lines) of different core configurations vs. pruning strength.}
    \label{fig:fig:flexsa_pe_util}
\end{figure}


\fig{fig:flexsa_pe_util_hbm} shows the impact on PE utilization and speedup using a single HBM2 for the DRAM system. Unlike the ideal memory BW case, this reflects the performance impact from GEMM tiling, input blocking, and wave scheduling. The 1G1C configuration shows 3\% reduced PE utilization on average across CNNs and pruning strengths compared to the results with ideal DRAM BW. This is because using a single 128$\times$128 GEMM maximizes in-core reuse, increasing math intensity per wave thus requiring low peak memory BW. The many-small cores configurations (1G4C and 4G4C) exhibit greater PE utilization decrease when memory BW is considered; the utilization drops by 9\% and 16\% for 1G4C and 4G4C, respectively. This PE utilization decrease is mainly caused by increased DRAM BW peaks from executing many small independent systolic waves in parallel. Not all inputs of these small systolic waves are coalesced thus the density of input loads is higher, which lowers overall memory BW utilization.

On the other hand, the two configurations using FlexSA show lower PE utilization drop compared to the naive many-core designs. This is because FlexSA uses small systolic waves only when using large waves hurts PE utilization. Furthermore, FlexSA offers two systolic array modes that use pairs of cores (VSW and HSW), which have higher in-core input reuse than using all cores fully independently. This helps balance PE utilization and input reuse. Overall, 1G1F improves average PE utilization by 33\% and 4\% compared to the 1G1C and 1G4C designs, respectively. The 4G1F configuration improves average PE utilization by 7\% compared to 4G4C. 
The increased PE utilization with FlexSA contributes to the overall performance improvement. 1G1F and 4F1FlexSA increase pruning while training speedup by the same degree of PE utilization compared to 1G4C and 4G4C configurations, which are shown by the speedup normalized to 1G1C (red line graphs in \fig{fig:flexsa_pe_util_hbm}).


\medskip
\noindent\textbf{On-chip Traffic and Energy Efficiency.}
Other than improving PE utilization, FlexSA reduces on-chip traffic by improving in-core input reuse. \fig{fig:flexsa_gbuf_loads} compares the average on-chip input traffic between the GBUF to LBUFs of convolution and FC layers using different models and core configurations. The red line graphs exhibit normalized traffics to the traffic of 1G1C. The naive many-core configurations (1G4C and 4G4C) increase the data traffic by 1.7$\times$ and 3.1$\times$, respectively, due to the reduced in-core reuse caused by using small independent systolic waves. On the other hand, the configurations using FlexSA show far lower data traffic compared to the naive many-core designs and similar traffic even compared to the design with larger cores. 1G1F reduces on-chip traffic by 41\% compared to 1G4C, and by 2\% even compared to 1G1C. This 2\% traffic saving comes from reusing the stationary inputs and outputs between multiple systolic waves in processing VSW and ISW modes, which is not possible with the baseline core design. 4G1F also saves on average 53\% GBUF traffic compared to 4G4C.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{graphs/gbuf_loads.pdf}
    \caption[On-chip traffic comparison]{On-chip traffic of different core configurations and pruning strengths.}
    \label{fig:flexsa_gbuf_loads}
\end{figure}


FlexSA reduces on-chip traffic and this improves the energy efficiency of training. To show this, we evaluate the dynamic energy consumed per training iteration using different core configurations (\fig{fig:energy_breakdown}). Each bar indicates the breakdown of energy consumed by different accelerator operations. \emph{COMP} indicates the energy consumed by mixed-precision multiply and accumulation operations of the FlexSA core. \emph{LBUF}, \emph{GBUF}, and \emph{DRAM} indicate the energy spent on data transmission associated with different resources. \emph{OverCore} indicates the over-core data transmission energy, which exists only in the configurations using FlexSA. The lines represent the energy increase compared to 1G1C. Because of the increased GBUF traffic, 1G4C and 4G4C exhibit $>$20\% total energy increase. The reason 4G4C shows similar energy compared to 1G4C though it requires higher traffic is that average global buffer access energy is lower with the distributed GBUFs. Both FlexSA configurations exhibit similar energy consumption as 1G1C. This high energy efficiency of FlexSA comes from using large systolic waves in most cases. The additional energy consumed by over-core data transmission is very small for all CNNs and pruning strengths.


\begin{figure}[t!]
    \centering                                                                            
    \subfloat[Medium pruning strength]{
        \includegraphics[width=0.48\textwidth]{graphs/energy_breakdown.pdf}
        \label{fig:energy_breakdown}
    }\\
    \vspace*{-2.0mm}
    \subfloat[High pruning strength]{
        \includegraphics[width=0.48\textwidth]{graphs/energy_breakdown2.pdf}
        \label{fig:energy_breakdown2}
    }
    \caption[Dynamic energy consumption comparison]{Breakdown of dynamic energy consumption per training iteration with different core configurations and pruning strength.}
    \label{fig:fig:flexsa_pe_util}
\end{figure}


\medskip
\noindent\textbf{FlexSA Operating Modes Breakdown.}
\fig{fig:inst_breakdown} shows the breakdown of FlexSA operating modes used in pruning while training using 1G1F and 4G1F. Each pie graph averages the results of ResNet50 and Inception v4 with different pruning strengths. This shows how frequently large systolic waves are used to improve in-core reuse and save energy consumption. For 1G1F, the FW accounts for 62\%, and VSW and HSW are used 23\% and 9\%, respectively.  For 4G1F, the ratio of using FW, VSW, and HSW increase to 83\%, 9\%, and 7\%, respectively. The lease efficient ISW accounts for only 6\% and 1\% for 1G1F and 4G1F. This result indicates that the inter-core operations of FlexSA are highly used to save on-chip BW and energy, and using only a restricted number of small independent systolic waves leads to high PE utilizations. Although not shown in the graph, Inception v4 shows slightly less FW utilization and greater VSW usage compared to ResNet50. This is because many convolution layers in the baseline Inception v4 network architecture have a small number of channels and are more energy- and PE utilization-efficiently executed with VSW. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{graphs/inst_breakdown.pdf}
    \caption[FlexSA modes selection breakdown]{FlexSA operating modes breakdown of pruning while training using 1G1F and 4G1F.}
    \label{fig:inst_breakdown}
\end{figure}




==> tex/test.tex <==
\section{Naive GEMM Core Splitting}
\label{sec:flexsa_core_splitting}

\medskip\noindent{\textbf{Diminishing PE Utilization and Increasing Input Load Cost.}}
The PE underutilization caused by small GEMM dimensions can be mitigated by splitting a large GEMM core into multiple small cores. However, this many-small-core design can be inefficient in processing typically large GEMM tiles, which account for most GEMM tiles in both pruned and unpruned CNN layers. First, small cores have low in-core input reuse compared to a large core, which increases input traffic from memory. Second, having more cores increases area complexity of wires, data path switches, and SRAM buffer control and decoding logic.

To observe the relation between the core size and PE utilization, I conduct a simple experiment that estimates overall PE utilization and the volume of on-chip input traffic while training ResNet50 using PruneTrain. The evaluation is done with different core configurations (\fig{fig:core_sweep}). Again, I use ideal memory BW to show the PE underutilization caused by the size mismatch between GEMM tiles and the core. The baseline accelerator design used in this experiment has a group of GEMM cores sharing a global buffer (GBUF) (\fig{fig:buffer_design}{.a}). The GBUF is used to block GEMM inputs. This baseline design also has a pair of local buffers (LBUFs) in each GEMM core for input double buffering to hide input load latency. The blue lines in \fig{fig:core_sweep} show PE utilizations and the red lines show average input traffic volume from the GBUF to LBUFs when using medium (plain lines) and high (dotted lines) pruning strengths. Both PE utilization and input traffic volume are averaged across training iterations over the whole training, thus they encapsulate the results of the baseline unpruned model and many different intermediate pruned models.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/buffer_design.pdf}
    \caption{Different GBUF configurations.}
    \label{fig:buffer_design}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{graphs/core_sweep.pdf}
    \caption[Impact of core sizing to PE utilization and GBUF loads]{PE utilization and GBUF load traffic increases for pruned ResNet50 training by splitting a single large core into many small cores. Medium and High indicate channel pruning strength.}
    \label{fig:core_sweep}
\end{figure}

